Directions for 3D User Interface Research from Consumer VR Games

With the continuing development of affordable immersive virtual reality (VR) systems, there is now a growing market for consumer content. The current form of consumer systems is not dissimilar to the lab-based VR systems of the past 30 years: the primary input mechanism is a head-tracked display and one or two tracked hands with buttons and joysticks on hand-held controllers. Over those 30 years, a very diverse academic literature has emerged that covers design and ergonomics of 3D user interfaces (3DUIs). However, the growing consumer market has engaged a very broad range of creatives that have built a very diverse set of designs. Sometimes these designs adopt findings from the academic literature, but other times they experiment with completely novel or counter-intuitive mechanisms. In this paper and its online adjunct, we report on novel 3DUI design patterns that are interesting from both design and research perspectives: they are highly novel, potentially broadly re-usable and/or suggest interesting avenues for evaluation. The supplemental material, which is a living document, is a crowd-sourced repository of interesting patterns. This paper is a curated snapshot of those patterns that were considered to be the most fruitful for further elaboration.

==> acknowledgements.tex <==
\section*{Acknowledgements}

We wish to thank Kyle Johnsen from University of Georgia who was involved in some of the early discussions about process. This process started when Anthony Steed was on a sabbatical visit to HIT Lab NZ at the University of Canterbury, New Zealand, supported by an Erskine Fellowship. Daniel Archer is supported by a Doctoral Training Partnership award from the UK's EPSRC. Tuukka M. Takala was supported by a Postdoctoral Fellowship of the Japan Society for the Promotion of Science.
